FewCLUE: A Chinese Few-shot Learning Evaluation Benchmark

Pretrained Language Models (PLMs) have achieved tremendous success in natural language understanding tasks. While different learning schemes -- fine-tuning, zero-shot, and few-shot learning -- have been widely explored and compared for languages such as English, there is comparatively little work in Chinese to fairly and comprehensively evaluate and compare these methods and thus hinders cumulative progress. In this paper, we introduce the Chinese Few-shot Learning Evaluation Benchmark (FewCLUE), the first comprehensive few-shot evaluation benchmark in Chinese. It includes nine tasks, ranging from single-sentence and sentence-pair classification tasks to machine reading comprehension tasks. We systematically evaluate five state-of-the-art (SOTA) few-shot learning methods (including PET, ADAPET, LM-BFF, P-tuning and EFL), and compare their performance with fine-tuning and zero-shot learning schemes on the newly constructed FewCLUE benchmark. Experimental results reveal that: 1) The effect of different few-shot learning methods is sensitive to the pre-trained model to which the methods are applied; 2) PET and P-tuning achieve the best overall performance with RoBERTa and ERNIE respectively. Our benchmark is used in the few-shot learning contest of NLPCC 2021. In addition, we provide a user-friendly toolkit, as well as an online leaderboard to help facilitate further progress on Chinese few-shot learning. We provide a baseline performance on different learning methods, a reference for future research.

==> Background.tex <==
\begin{figure*}[t]
	\centering
	\includegraphics[width=1.0\textwidth]{./pictures/inconsistency_construction.pdf}
	\caption{
		The process of CI-ToD construction.}
	\label{fig:construction-step}
\end{figure*}


\begin{figure}[t]
	\centering
	\includegraphics[scale=0.5]{./pictures/Inconsistency_type.pdf}
	\caption{
		Inconsistent types in CI-ToD. Different colors denote different inconsistent types.
	}
	\label{Inconsistency type}
\end{figure}

\begin{figure*}[t]
	\centering
	\includegraphics[width=0.9\linewidth]{./pictures/annotation.pdf}
	\caption{
		The collection interface.
	}
	\label{annotation interface}
\end{figure*}

In our paper, the consistency identification in task-oriented dialogue is formulated as a supervised multi-label classification task, which aims to judge whether the generated system response is inconsistent.
To equip the model with the ability to analyze what the inconsistent sources lead to it, we require the model not only provide the final prediction but also the fine-grained sources including dialogue history, knowledge base (KB) and user's query.
More specifically, given a task-oriented dialogue between a user ($u$) and a system ($s$), the $n$-turned dialogue snippet consists of dialogue history $H$ = $\{(u_{1}, s_{1} ), (u_{2} , s_{2} ), ... , (u_{n-1} , s_{n-1} )\}$, the corresponding knowledge base $KB$, the user query $u_{n}$ and system response $s_{n}$.
More specifically, the task can be defined as:
\begin{eqnarray}
		\mathbf{y} = f ([H, KB, u_{n}], s_{n}), 
\end{eqnarray}
where $f$ denotes the trainable model; $\mathbf{y}$ is an output three-dimension vector, indicating whether the last utterance $s_{n}$ contradicts any previously mentioned dialogue history $H$, user query $u_{n}$ or the corresponding knowledge base $KB$ .

